Learning Controller Gains on Bipedal Walking Robots via User Preferences

Experimental demonstration of complex robotic behaviors relies heavily on finding the correct controller gains. This painstaking process is often completed by a domain expert, requiring deep knowledge of the relationship between parameter values and the resulting behavior of the system. Even when such knowledge is possessed, it can take significant effort to navigate the nonintuitive landscape of possible parameter combinations. In this work, we explore the extent to which preference-based learning can be used to optimize controller gains online by repeatedly querying the user for their preferences. This general methodology is applied to two variants of control Lyapunov function based nonlinear controllers framed as quadratic programs, which provide theoretical guarantees but are challenging to realize in practice. These controllers are successfully demonstrated both on the planar underactuated biped, AMBER, and on the 3D underactuated biped, Cassie. We experimentally evaluate the performance of the learned controllers and show that the proposed method is repeatably able to learn gains that yield stable and robust locomotion.

==> Sections/Intro_Maegan.tex <==
\section{Introduction} \label{sec:intro}


Bipedal locomotion is a challenging yet well-explored area of research. Some of the biggest challenges in bipedal locomotion include how to account for compliance, under-actuation, and external disturbances. Achieving stable and robust experimental walking with the 3D bipedal robot Cassie requires tackling all of these challenges. There are many previously demonstrated approaches towards achieving stable and robust walking on Cassie [cite a few Cassie papers here]. Most recently, [Jenna's paper] introduced the first demonstration of an ID-CLF-QP on Cassie. 

CLF-QPs were first introduced in ...... and have since become popular in the control community because of their formal theoretical guarantees. However, in practice these controllers are extremely challenging because they have several (~60?) parameters that need to be hand tuned. Most of this hand-tuning arises from unknown differences between the physical robot and the robot model. Furthermore, this parameter landscape is often non-intuitive and requires dedicated time even for domain experts (in [Jenna's paper] about 2?? months was spent tuning parameters). 

\textcolor{red}{The controllers have theoretical guarantees, but in practice it always comes down to parameter tuning}

\textcolor{red}{The landscape of parameters to tune is often non-intuitive and requires significant time, even for domain experts}

\red{talk about learning and control. End to end, one piece. Then mention how this is a different paradigm, using the user}

\textcolor{red}{By navigating through the Bayesian landscape of the preferences of practitioners, we are able to navigate towards behavior that works on hardware}. Previous work has demonstrated alternative methods of selecting heuristic parameters such as controller gains [cite other examples here]. In particular, \cite{tucker2020preferencebased} introduced the use of preference-based learning towards selecting essential constraints of an HZD gait generation framework which resulted in stable and robust experimental walking on a planar biped with unmodeled compliance at the ankle. Preferences are particularly beneficial because they are able to capture the notion of ``general goodness'' that is often sought after during parameter tuning. 

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.675\linewidth]{Figures/KungFuCassie.png}
    \caption{A depiction of the Cassie robot.}
    \label{fig:cassie}
\end{figure}


Inspired by the success of preference-based learning towards tuning gait parameters, we applied a similar learning framework towards learning gains of a ID-CLF-QP controller on the Cassie biped robot. This application required extending the learning framework to a much higher-dimensional space which led to some unique challenges. First, more user feedback was required to navigate the larger action space. This was accomplished by sampling actions continuously on hardware which led to a much faster rate of obtaining feedback. Second, to increase the speed of the learning, ordinal labels were also added as a feedback mechanism. However to avoid obtaining noisy labels, the ordinal feedback was limited to only three categories: very bad, neutral, and very good. 

In this paper, we briefly present the control and learning frameworks in Sections \ref{sec:opt} and \ref{sec:framework} respectively. We then present the results of the experiments in Section \ref{sec:exp} where we evaluate the performance of the controller with the learned gains as well as the duration of time it took to find the optimal gains. Finally, we conclude with Section \ref{sec:conc}. Overall, the results of this paper indicate that preference-based learning is an effective method towards tuning control parameters.

Bayesian optimization is a probabilistic approach towards identifying $a^* = \argmax_a f(a)$ for some unknown utility function $f(a): a \to \R$ evaluated over individual actions $a \in \A$. Typically, Bayesian optimization is used on problems where $f(a)$ is difficult to evaluate but can be obtained. However, recent work extended Bayesian optimization to the preference setting \cite{sui2018advancements}, where instead of obtaining $f(a)$ for each sampled action $a$, only pairwise preferences between sampled actions are sequentially obtained. We refer to this setting as ``preference-based learning''. In this work, we utilize a more recent preference-based learning algorithm, LineCoSpar \cite{tucker2020human} with the addition of ordinal labels inspired from \cite{li2020roial}. The resulting learning framework iteratively applies Thompson sampling to navigate a high-dimensional Bayesian landscape of user preferences. 


As opposed to tuning PD gains, tuning the parameters in a Control Lyapunov function can be significantly less intuitive and more challenging. This method does not rely on domain expertise to tune parameters, and instead allows even a na\"ive user to go from stumbling to walking in a matter of a few hours. 

==> Sections/Intro_Take2.tex <==
\section{Introduction} \label{sec:intro}

Achieving robust and stable performance for physical robotic systems relies heavily on careful gain tuning, regardless of the implemented controller. 
Significant effort has been dedicated to the art of parameter tuning, with detailed accounts of ways to tune PID gains and CLF gains \red{cite?}.
Recently, machine learning techniques have been implemented to alleviate the process of hand-tuning gains by systematically navigating the entire parameter space \cite{birattari2009tuning,jun1999automatic,marco2016automatic}. However, these techniques rely on a carefully constructed predefined reward function. Moreover, it is often the case where different desired properties of the robotic behavior are conflicting such that they both can't be optimized simultaneously. In our work, we propose the use of preference-based learning to tune control parameters, which relies only on subjective user feedback, mainly pairwise preferences, eliminating the need for a reward function.

Controller gains for bipedal locomotion are particularly difficult to tune due to extreme sensitivity of the controller parameters on stability. Other challenges in achieving bipedal locomotion include how to account for compliance, under-actuation, and external disturbances. Achieving stable and robust experimental walking with the 3D bipedal robot Cassie requires tackling all of these challenges. Recently, \red{[Jenna's paper]} introduced the first demonstration of a variant of the control Lyaponov function quadratic program controller (ID-CLF-QP$^+$) on Cassie. 

ID-CLF-QP$^+$ has demonstrated excellent performance to tackle the problem of bipedal locomotion. Concomitantly, tuning the parameters in a Control Lyapunov function can be significantly less intuitive and more challenging than tuning PD gains. The learning method we present does not rely on domain expertise to tune parameters, and instead allows even a na\"ive user to go from stumbling to walking in a matter of a few hours. 

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.652\linewidth]{Figures/KungFuCassie.png}
    \caption{A depiction of the Cassie robot.}
    \label{fig:cassie}
\end{figure}

It was shown in \cite{ames2013towards} that control Lyapunov functions could stabilize locomotion through the hybrid zero dynamics framework, with \cite{galloway2015torque} demonstrating how this can be implemented as a quadratic program to allow the problem to be solved in the face of feasibility constraints in a pointwise-optimal fashion. The resulting control Lyaponov function quadratic program (CLF-QP) controller has since become popular in the control community because of their formal theoretical guarantees \cite{ nguyen2016exponential} \red{need more cites here}. However, in practice these controllers are extremely challenging because they have several (~60?) parameters that need to be hand tuned. Most of this hand-tuning arises from unknown differences between the physical robot and the robot model. Furthermore, this parameter landscape is often non-intuitive and requires dedicated time even for domain experts (in [Jenna's paper] about 2?? months was spent tuning parameters). 

\textcolor{red}{The controllers have theoretical guarantees, but in practice it always comes down to parameter tuning}

\textcolor{red}{The landscape of parameters to tune is often non-intuitive and requires significant time, even for domain experts}

\red{talk about learning and control. End to end, one piece. Then mention how this is a different paradigm, using the user}




\textcolor{red}{By navigating through the Bayesian landscape of the preferences of practitioners, we are able to navigate towards behavior that works on hardware}.  In particular, \cite{tucker2020preferencebased} introduced the use of preference-based learning towards selecting essential constraints of an HZD gait generation framework which resulted in stable and robust experimental walking on a planar biped with unmodeled compliance at the ankle. Preferences are particularly beneficial because they are able to capture the notion of ``general goodness'' that is often sought after during parameter tuning. Inspired by the success of preference-based learning for selecting walking gaits, we applied a similar learning framework towards learning gains of a ID-CLF-QP controller on the Cassie biped robot. This application required extending the learning framework to a much higher-dimensional space which led to some unique challenges. First, more user feedback was required to navigate the larger action space. This was accomplished by sampling actions continuously on hardware which led to a much faster rate of obtaining feedback. Second, to increase the speed of the learning, ordinal labels were also added as a feedback mechanism. However to avoid obtaining noisy labels, the ordinal feedback was limited to only three categories: very bad, neutral, and very good. 


This paper is structured as follows: Sections \ref{sec:opt} and \ref{sec:framework} briefly introduce the control and learning frameworks, respectively. Section \ref{sec:exp} demonstrates the results of the experiments, wherein we evaluate the duration of time it took to find the optimal gains, as well as the performance of the controller with the learned gains. Finally, Section \ref{sec:conc} provides closing remarks. 

Overall, the results of this paper indicate that preference-based learning is an effective method towards tuning control parameters.






==> Sections/Intro_messy.tex <==
\section{Introduction} \label{sec:intro}

\red{Current flow: Tuning gains is difficult for Cassie. CLF-QPs are good controllers to acheive stable robust locomotion on 3D bipeds. CLF-QPs are unintuitive to tune. Machine Learning can be used to navigate parameter landscapes. We propose using preference-based learning to avoid defining a reward function. }

\red{Maegan proposed flow: Achieving stable locomotion on robots with complex dynamics and underactuation is particularly difficult. Moreover, achieving robust behavior in the presence of external disturbances requires a real-time controller. CLF-QPs have recently shown to be successful at acheiving stable and robust locomotion on Cassie. However, CLF-QPs are difficult to implement on hardware because they have many control parameters and are unintuitive to tune. A potential solution is to utilize machine learning which can navigate parameter landscapes. However, machine learning requires defining a reward function which is difficult for complex behaviors such as 3D bipedal locomotion. We propose using preference-based learning to avoid defining a reward function. }

\red{New Flow: Behavior relies on controller gains. Navigating this space is hard even for domain experts. Becomes even harder for more complicated controllers. But these complicated controllers are necessary for complicated robots. Cassie is especially hard because you need complicated controllers, but this makes the gain tuning process tedious and difficult. To alleviate the gain tuning process and enable the use of complicated controllers for na\"ive users, we propose preference-based learning to achieve stable and robust walking on Cassie.}

\blue{Achieving robust and stable performance for physical robotic systems relies heavily on careful gain tuning, regardless of the implemented controller. Navigating the space of possible parameter combinations is a challenging endeavor, even for domain experts. To combat this challenge, many people have developed systematic ways to tune parameters for specific controller types \red{cite}. For controllers where the input/output relationship between parameters and the resulting behavior is less clear, this can be prohibitively difficult. These difficulties are especially prevalent in the setting of 3D bipedal locomotion, due to extreme sensitivity of the stability of the system with respect to controller parameters.}

\blue{
% Stable walking can be achieved through the construction of stabilizing controllers.
It was shown in \cite{ames2013towards} that control Lyapunov functions are capable of stabilizing locomotion through the hybrid zero dynamics framework, with \cite{galloway2015torque} demonstrating how this can be implemented as a quadratic program to allow the problem to be solved even in the face of feasibility constraints in a pointwise-optimal fashion. Achieving robust walking behavior on the 22 degree of freedom (DOF) Cassie biped is particularly difficult due to compliance in the legs, under-actuation at the feet, and a narrow domain of attraction. One such controller that has recently been demonstrated to achieve stable locomotion on Cassie is a variant of the control Lyapunov function quadratic program (CLF-QP), termed the ID-CLF-QP$^+$ [Cite Jenna].}
\blue{

However, synthesizing a controller which can account for the complexities of 3D locomotion necessitates the addition of numerous control parameters, exacerbating the issue of gain tuning. 

For example, implementing the ID-CLF-QP$^+$ requires hand-tuning (~60?) parameters. Most of this hand-tuning arises from unknown differences between the physical robot and the robot model. This parameter landscape is non-intuitive and requires dedicated time even for domain experts (in [Jenna's paper] about 2?? months was spent tuning parameters).

Recently, machine learning techniques have been implemented to alleviate the process of hand-tuning gains in a controller agnostic way by systematically navigating the entire parameter space \cite{birattari2009tuning,jun1999automatic,marco2016automatic}. However, these techniques rely on a carefully constructed predefined reward function. Moreover, it is often the case where different desired properties of the robotic behavior are conflicting such that they both can't be optimized simultaneously. In our work, we propose the use of preference-based learning to tune control parameters, which relies only on subjective user feedback, mainly pairwise preferences, eliminating the need for a reward function.
}

\textcolor{red}{By navigating through the Bayesian landscape of the preferences of practitioners, we are able to navigate towards behavior that works on hardware}.  In particular, \cite{tucker2020preferencebased} introduced the use of preference-based learning towards selecting essential constraints of an HZD gait generation framework which resulted in stable and robust experimental walking on a planar biped with unmodeled compliance at the ankle. Preferences are particularly beneficial because they are able to capture the notion of ``general goodness'' that is often sought after during parameter tuning. Inspired by the success of preference-based learning for selecting walking gaits, we applied a similar learning framework towards learning gains of a ID-CLF-QP controller on the Cassie biped robot. This application required extending the learning framework to a much higher-dimensional space which led to some unique challenges. First, more user feedback was required to navigate the larger action space. This was accomplished by sampling actions continuously on hardware which led to a much faster rate of obtaining feedback. Second, to increase the speed of the learning, ordinal labels were also added as a feedback mechanism. However to avoid obtaining noisy labels, the ordinal feedback was limited to only three categories: very bad, neutral, and very good. 

This paper is structured as follows: Sections \ref{sec:opt} and \ref{sec:framework} briefly introduce the control and learning frameworks, respectively. Section \ref{sec:exp} demonstrates the results of the experiments, wherein we evaluate the duration of time it took to find the optimal gains, as well as the performance of the controller with the learned gains. Finally, Section \ref{sec:conc} provides closing remarks. 

% Overall, the results of this paper indicate that preference-based learning is an effective method towards tuning control parameters.



% Overall, the point we are trying to make is that complicated controllers (such as the ID-CLF-QP$^+$) with numerous control parameters are necessary to achieving stable locomotion. The current solution to htis problem is to have a domain expert spend many months tuning these paraters to acheive stable locomotin. We propose pref-based leraning.} 



% Complicated controllers with many control parameters are often necessary in order to achieve ideal behavior. This is especially the case for achieving stable locomotion on 3D bipeds, due to complexities such as compliance, under-actuation, model uncertainty, external disturbances.

% The construction of a stabilizing controller is an especially hard problem in the setting of bipedal locomotion, and is even more prevalent for 3D bipedal robots with under-actuation.

% However, synthesizing a controller which can account for the complexities of 3D locomotion, especially in the presence of compliance, under-actuated behavior, and external disturances, such as the 22 degree of freedom (DOF) Cassie robot, necessitates the addition of numerous control parameters. 

% under-actuation and compliance in the legs, while being robust to external disturbance

% Controller gains for bipedal locomotion are particularly difficult to tune due to extreme sensitivity of the stability of the system with respect to controller parameters. The issue of stability is even more prevalent for 3D bipedal robots with under-actuation, such as the 22 degree of freedom (DOF) Cassie robot. 
% Constructing a controller which can account for this under-actuation, as well as compliance in the legs, while being robust to external disturbance necessitates the addition of numerous control parameters.

% It was shown in \cite{ames2013towards} that control Lyapunov functions could stabilize locomotion through the hybrid zero dynamics framework, with \cite{galloway2015torque} demonstrating how this can be implemented as a quadratic program to allow the problem to be solved in the face of feasibility constraints in a pointwise-optimal fashion. 

% However, the CLF-QP has many parameters. 

% One such controller that has recently been demonstrated to achieve stable and robust behavior on Cassie is a variant of the control Lyapunov function quadratic program [Cite Jenna]. 


% The resulting control Lyaponov function quadratic program (CLF-QP) controller has since become popular in the control community because of their formal theoretical guarantees \cite{ nguyen2016exponential} \red{need more cites here}. 

% is tightly coupled to the choice of controller gains. 


% Moreover, under-actuated bipedal robots are especially difficult to tune since the stability of the robot is a product of many factors of the walking.

% The issue of stability is even more prevalent for 3D bipedal robots with under-actuation, such as the 22 degree of freedom (DOF) Cassie robot. 
% Achieving stable and robust walking on Cassie requires selecting parameters which can account for under-actuation, compliance in the legs, and external disturbances. 
% Other challenges in achieving bipedal locomotion include how to account for
%  requires tackling all of these challenges.

% Recently, \red{[Jenna's paper]} introduced the first demonstration of a variant of the control Lyaponov function quadratic program controller (ID-CLF-QP$^+$) on Cassie. ID-CLF-QP$^+$ has demonstrated excellent performance to tackle the problem of bipedal locomotion. 
% However, in practice these controllers are extremely challenging because they have several (~60?) parameters that need to be hand tuned. Most of this hand-tuning arises from unknown differences between the physical robot and the robot model. Furthermore, this parameter landscape is often non-intuitive and requires dedicated time even for domain experts (in [Jenna's paper] about 2?? months was spent tuning parameters). 

% Navigating the space of possible parameter combinations is a challenging endeavor, even for domain experts, and many people have developed systematic ways to achieve this for specific controller types \red{cite}. Recently, machine learning techniques have been implemented to alleviate the process of hand-tuning gains in a controller agnostic way by systematically navigating the entire parameter space \cite{birattari2009tuning,jun1999automatic,marco2016automatic}. However, these techniques rely on a carefully constructed predefined reward function. Moreover, it is often the case where different desired properties of the robotic behavior are conflicting such that they both can't be optimized simultaneously. In our work, we propose the use of preference-based learning to tune control parameters, which relies only on subjective user feedback, mainly pairwise preferences, eliminating the need for a reward function.




% Tuning the parameters in a Control Lyapunov function can be significantly less intuitive and more challenging than tuning PD gains. The learning method we present does not rely on domain expertise to tune parameters, and instead allows even a na\"ive user to go from stumbling to walking in a matter of a few hours. 

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.652\linewidth]{Figures/KungFuCassie.png}
    \caption{A depiction of the Cassie robot.}
    \label{fig:cassie}
\end{figure}



% \textcolor{red}{The controllers have theoretical guarantees, but in practice it always comes down to parameter tuning}

% \textcolor{red}{The landscape of parameters to tune is often non-intuitive and requires significant time, even for domain experts}

% \red{talk about learning and control. End to end, one piece. Then mention how this is a different paradigm, using the user}



% Significant effort has been dedicated to the art of parameter tuning, with detailed accounts of ways to tune PID gains and CLF gains \red{cite?}.










==> Sections/outline.tex <==
Goal of our work is to explore the use of prefernece-based leraning towards tuning a CLF-QP.

CLF-QPs have been implemented only on few platforms - in part due to their difficultly in tuning. However, the reason to use CLF's despite their difficulty is because they have all of these benefits compared to PD controllers [cite theory papers] and you can put them in a QP. Introduce CLF-QP. 

How are CLF-QPs typically tuned: using the Q matrix. Brief discussion about why tuning Q matrix is non intuitive. 


AMBER:
too low - AMBER collapses - artificially driving V to zero. Vdot only has to be slightly negative - robot collapses.

too high - torque chatter?

feed forward torque from trajectory optimization?


For harder systems you need to do a more complicated CLF-QP. Introduce ID-CLF-QP.


Typically CLF-Qps are tuned by ...... 
